Trust Assessment in Online Social Networks

Assessing trust in online social networks (OSNs) is critical for many applications such as online marketing and network security. It is a challenging problem, however, due to the difficulties of handling complex social network topologies and conducting accurate assessment in these topologies. To address these challenges, we model trust by proposing the three-valued subjective logic (3VSL) model. 3VSL properly models the uncertainties that exist in trust, thus is able to compute trust in arbitrary graphs. We theoretically prove the capability of 3VSL based on the Dirichlet-Categorical (DC) distribution and its correctness in arbitrary OSN topologies. Based on the 3VSL model, we further design the AssessTrust (AT) algorithm to accurately compute the trust between any two users connected in an OSN. We validate 3VSL against two real-world OSN datasets: Advogato and Pretty Good Privacy (PGP). Experimental results indicate that 3VSL can accurately model the trust between any pair of indirectly connected users in the Advogato and PGP.

==> content/other.tex <==
\section{Introduction}  

Online Social Networks (OSNs) help people not only to strengthen their connections with known friends, but also to expand their social circle to friends of friends that they may not know previously.\\
%

One the other hand, the development of OSNs is also associated with the rise of OSNs spam attack. 
%
Therefore, OSNs spammer detection has attracted many attentions in recent years
%
Many previous efforts have been devoted to this problem~\cite{kim2012oto, yu2008sybilguard}. 
%
The basic principle of most previous work  is finding friend communities inside a social network and treating the nodes outside the community as suspicious users.  
%
However, recent studies~\cite{6547122} indicate that using topological information only to detect a friend community is not sufficient to identify spammers.
%
For example, many spammers pretend to be a normal user and broadcast friend requests in OSNs. 
%
They can be identified as a member of the community as long as few of their requests are accepted.\\   
%

In view of this limitation, we make use of trust in OSNs to identify spammers. 
%
The basic principle is that a friend's friend is trustworthy while an user whom my friends barely have interaction with is suspicious.
%
The assumption behind this idea is that normal users will never have strong social ties (messages, likes, ratings, etc.) with spammers, even though there is an edge between them.
%
In our previous work~\cite{6848107}, we proposed a trust model called 3VSL to assess the trustworthiness of a strange user in OSNs by propagating trust along the social ties among friends.      
%
3VSL defines trust as a \textit{probability} that a trustee will behave good as expected by a trustor. 
%
Such probability, which is called opinion, is expressed as a Dirichlet-Categorical distribution. 
%
Through aggregating and propagating opinions in OSNs, 3VSL is able to assess the trustworthiness of target users and identify spammers.  \\
%

A problem remaining to 3VSL is how to estimate the factors of an opinion. 
%
In other words, how to map social tie features such as messages, likes, ratings to the factors of Dirichlet-Categorical distribution, such that 3VSL model can give accurate result for spammer detection? Formally, we define the system model as followings:\\

\textit{A social interaction network is modeled as a feature matrix $V$ where an entry $V_{ij}$ is a feature vector $V_{ij}$. 
%
The feature vector $V_{ij}$ is composed of features collected from the interactions between user $i$ and $j$ on OSNs.
%
An opinion network is modeled as an opinion matrix $O$, where an entry $O_{ij}$ is an opinion from user $i$ to $j$.
%
The opinion is a tuple of factors expressing a certain Dirichlet-Categorical distribution.} \\
%

Then, the problem is formulated as:\\

%
\textit{Given a feature matrix $V$, how to estimate the opinion matrix $O$, upon which 3VSL model is able to conduct an accurate trust assessment for spammer detection.} 


==> figure/IEEEtran/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************

